Large Interferometer For Exoplanets (LIFE): VI. Detecting rocky exoplanets in the habitable zones of Sun-like stars

While previous studies have shown a strong preference for a future mid-infrared nulling interferometer space mission to detect planets within the HZ around M dwarfs, we here focus on a more conservative approach toward the concept of habitability and present yield estimates for two stellar samples consisting of nearby (d<20 pc) Sun-like stars (4800-6300 K) and nearby FGK-type stars (3940-7220 K) accessible to such a mission. Our yield estimates are based on recently derived occurrence rates of rocky planets from the Kepler mission and our LIFE exoplanet observation simulation tool LIFEsim, which includes all main astrophysical noise sources, but no instrumental noise sources as yet. Depending on a pessimistic or optimistic extrapolation of the Kepler results, we find that during a 2.5-year search phase, LIFE could detect between ~10-16 (average) or ~5-34 (including 1$\sigma$ uncertainties) rocky planets (0.5-1.5 R${}_\rm{Earth}$) within the optimistic HZ of Sun-like stars and between ~4-6 (average) or ~1-13 (including 1$\sigma$ uncertainties) exo-Earth candidates (EECs) assuming four collector spacecraft equipped with 2 m mirrors and a conservative instrument throughput of 5%. With D=3.5 m or 1 m mirrors, the yield $Y$ changes strongly, following approximately $Y \propto D^{3/2}$. With the larger sample of FGK-type stars, the yield increases to ~16-22 (average) rocky planets within the optimistic HZ and ~5-8 (average) EECs. Furthermore, we find that in addition to the mirror diameter, the yield depends strongly on the total throughput, but only weakly on the exozodiacal dust level and the accessible wavelength range of the mission. When the focus lies entirely on Sun-like stars, larger mirrors (~3 m with 5% total throughput) or a better total throughput (~20% with 2 m mirrors) are required to detect a statistically relevant sample of ~30 rocky planets within the optimistic HZ.

==> biblatex.tex <==

%!TEX root = ../main.tex

% -----------------------------------------------------------------------------
% Load BibLaTeX with various options
\usepackage[abbreviate=false,
            backend=biber,
            citetracker=true,
            dashed=false,
            doi=true,
            giveninits=true,
            maxbibnames=3,
            maxcitenames=2,
            sorting=nyt,
            style=authoryear-comp,
            sortcites=false,
            urldate=long,
            uniquename=false,
            uniquelist=false]{biblatex}

% Do not print month or day of the publication
\AtEveryBibitem{\clearfield{month}}
\AtEveryBibitem{\clearfield{day}}

% Increase spacing between items in bibliography
\setlength\bibitemsep{1.75\itemsep}

% Remove the "In:" before the journal title and replace it with a full stop
\renewbibmacro{in:}{%
  \ifentrytype{article}{}{\printtext{\bibstring{in}\intitlepunct}}}

% Don't put a "p." before the page numbers in an entry
\DeclareFieldFormat[article]{pages}{#1}

% Print articles as:
%     Journal Title, Issue(Number): Pages
% instead of:
%    Journal Title, Issue.Number: Pages
\renewcommand\bibpagespunct{\ifentrytype{article}{\addcolon}{\addcomma}\space}
\renewbibmacro*{volume+number+eid}{%
  \printfield{volume}%
  \printfield[parens]{number}%
  \setunit{\addcomma\space}%
  \printfield{eid}}

% Define how links are displayed for arXiv papers
\DeclareFieldFormat*{eprint:arxiv}{%
  \ifhyperref
    { \href{http://arxiv.org/abs/#1}{\nolinkurl{arXiv:#1}} }
    { \nolinkurl{arXiv:#1} }
}


% Add the comma between the journal title and the issue / number
\usepackage{xpatch}
\xpatchbibmacro{journal+issuetitle}{%
  \setunit*{\addspace}%
  \iffieldundef{series}}
  {%
  \setunit*{\addcomma\space}%
  \iffieldundef{series}}{}{}


% Adjust the format of the backreferences
\DefineBibliographyStrings{english}{%
    backrefpage  = {\lowercase{c}ited on p.},
    backrefpages = {\lowercase{c}ited on pp.}
}

% Make sure that the whole citation entry, e.g. "(Smith, 2000)", is a link to
% the bibliography, and not just the year.
% Source: https://tex.stackexchange.com/a/27107/97669
\DeclareFieldFormat{citehyperref}{%
  \DeclareFieldAlias{bibhyperref}{noformat}% Avoid nested links
  \bibhyperref{#1}}
\DeclareFieldFormat{textcitehyperref}{%
  \DeclareFieldAlias{bibhyperref}{noformat}% Avoid nested links
  \bibhyperref{%
    #1%
    \ifbool{cbx:parens}
      {\bibcloseparen\global\boolfalse{cbx:parens}}
      {}}}
\savebibmacro{cite}
\savebibmacro{textcite}
\renewbibmacro*{cite}{%
  \printtext[citehyperref]{%
    \restorebibmacro{cite}%
    \usebibmacro{cite}}}
\renewbibmacro*{textcite}{%
  \ifboolexpr{
    ( not test {\iffieldundef{prenote}} and
      test {\ifnumequal{\value{citecount}}{1}} )
    or
    ( not test {\iffieldundef{postnote}} and
      test {\ifnumequal{\value{citecount}}{\value{citetotal}}} )
  }
    {\DeclareFieldAlias{textcitehyperref}{noformat}}
    {}%
  \printtext[textcitehyperref]{%
    \restorebibmacro{textcite}%
    \usebibmacro{textcite}}}


==> preamble/commands.tex <==

%!TEX root = ../main.tex


% Commands for "e.g." and "i.e."
\newcommand{\eg}{e.g.,~}
\newcommand{\ie}{i.e.,~}

% Commands for all authors
\newcommand{\tg}[1]{{\color{RedOrange}\textbf{[TG]}~#1}}
\newcommand{\mb}[1]{{\color{ForestGreen}\textbf{[MB]}~#1}}
\renewcommand{\sq}[1]{{\color{NavyBlue}\textbf{[SQ]}~#1}}
\newcommand{\bs}[1]{{\color{Purple}\textbf{[BS]}~#1}}

% A customized \todo command
\newcommand{\todo}[1]{{\color{Red}\textbf{[todo]}~#1}}

% A customized \idea command
\newcommand{\idea}[1]{{\color{Dandelion}\textbf{[idea]}~#1}}

% A customized \checkthis command
\newcommand{\checkthis}[1]{{\color{HotPink}\textbf{#1}}}

% Shortcut for bold math symbols
\newcommand{\bms}[1]{\boldsymbol{#1}}

% Symbol for "causally independent"
\newcommand{\indep}{\protect\rotatebox[origin=c]{90}{$\vDash$}}

% Circled numbers
\newcommand{\circled}[1]{\textcircled{\raisebox{-0.4pt}{\tiny#1}}}


\newcommand{\textcite}{\citet}
\newcommand{\parencite}{\citep}

==> preamble/crossref.tex <==

%!TEX root = ../main.tex

% -----------------------------------------------------------------------------

% Load hyperref
\usepackage[pdftex,
            unicode=true,
            colorlinks,
            urlcolor=Blue,
            linkcolor=gray,
            citecolor=gray,
            filecolor=gray,
            pdfauthor={Timothy Gebhard},
            plainpages=false,
            pdfpagelabels]{hyperref}

% Avoid "hyperref Warning: Suppressing link with empty target".
% Source: https://tex.stackexchange.com/a/345918/97669
\makeatletter
\renewcommand*\aa@pageof{, page \thepage{} of \pageref*{LastPage}}
\makeatother

% -----------------------------------------------------------------------------

% Load cleverref
% Allows "smart" referencing using the \cref{} command
\usepackage[noabbrev]{cleveref}

% According to the Chicago Manual of Style:
%   "The words chapter, part, appendix, table, figure, and the like are
%   lowercased and spelled out in text (though sometimes abbreviated in
%   parenthetical references).%
% We load cleveref without abbreviations as a default, and then define a
% \cshrf{} command that will give the abbreviated form.
\DeclareRobustCommand{\abbrevcrefs}{%
    \crefname{figure}{fig.}{figs.}%
    \crefname{equation}{eq.}{eqs.}%
}
\DeclareRobustCommand{\cshref}[1]{{\abbrevcrefs\cref{#1}}}

% -----------------------------------------------------------------------------

% Load url
% To correctly typeset hyperlinks with \url{}
\usepackage{url}

% -----------------------------------------------------------------------------

% Define \spliturl{}{} command to allow to split URL over two lines within the
% LaTeX code (to avoid long lines in the source code!)

\newcommand{\spliturl}[2]{\url{#1#2}}

% -----------------------------------------------------------------------------

% Fix positioning of links to captions
\usepackage[all]{hypcap}


==> preamble/figures.tex <==

%!TEX root = ../main.tex

% -----------------------------------------------------------------------------
% FIGURE ENVIRONMENTS IN GENERAL
% -----------------------------------------------------------------------------

% Load float
% "Advanced" floating: [H] forces an element to be positioned exactly at the
% given position. However, this is usually not recommended.
\usepackage{float}


% -----------------------------------------------------------------------------
% GRAPHICS
% -----------------------------------------------------------------------------

% Include and rotate graphics
\usepackage{graphicx}
\usepackage{rotating}

\usepackage{silence}
\WarningFilter{caption}{Unknown document class}
\usepackage{subcaption}


% -----------------------------------------------------------------------------
% TABLES
% -----------------------------------------------------------------------------

% The default package for more professional tables
\usepackage{booktabs}

% Needed for the \adjincludegraphics command
\usepackage{adjustbox}


% The option 'C' with tabularx gives a centered column with automatic
% column balancing
\usepackage{tabularx}
\newcolumntype{C}{>{\centering\arraybackslash}X}


% Merge not only columns, but also rows
\usepackage{multirow}


% Also create tables that span more than a single page
\usepackage{longtable}


==> preamble/miscellaneous.tex <==

%!TEX root = ../main.tex

% -----------------------------------------------------------------------------

% Dummy text generators
\usepackage{lipsum}
\usepackage{kantlipsum}

% -----------------------------------------------------------------------------

% For multi-line comments
\usepackage{verbatim}


==> preamble/pagestyles.tex <==

%!TEX root = ../main.tex

% -----------------------------------------------------------------------------

% Datetime package to print the draft time
% \usepackage[showzone=false]{datetime2}

% Get more control over titlepage
\usepackage{titling}
\usepackage{authblk}

% Clear empty pages (no page numbers etc.)
\usepackage{emptypage}

% -----------------------------------------------------------------------------

\pretitle{\begin{center}\bfseries\LARGE}  %\sffamily
\posttitle{\end{center}}

\renewcommand\Affilfont{\small\itshape}

% -----------------------------------------------------------------------------

% Define main page style
\nouppercaseheads
\makepagestyle{main}
\makeheadrule {main}{\textwidth}{\normalrulethickness}
\makefootrule {main}{\textwidth}{\normalrulethickness}{\footruleskip}
\makeevenhead {main}{}{\shortauthor:~\shorttitle}{}
\makeoddhead  {main}{}{\shortauthor:~\shorttitle}{}
\makeevenfoot {main}{}{\thepage}{}
\makeoddfoot  {main}{}{\thepage}{}
\makeatletter % because of \@chapapp
\makepsmarks {main}{
    \createmark {chapter} {both} {shownumber}{\@chapapp\ }{: \ }
    \createmark {section} {right}{shownumber}{} {. \ }
}
\makeatother
\setsecnumdepth{section}

% -----------------------------------------------------------------------------

% Define the "first page" page style
\makepagestyle{plain}
\makefootrule {plain}{\textwidth}{\normalrulethickness}{\footruleskip}
\makeevenfoot {plain}{}{\thepage}{}
\makeoddfoot  {plain}{}{\thepage}{}

% -----------------------------------------------------------------------------

\usepackage{etoolbox}
\patchcmd{\maketitle}{plain}{firstpage}{}{}

% -----------------------------------------------------------------------------

% Adjust sizes of headings for sections, subsections and subsubsections
\setsecheadstyle{\Large\bfseries}
\setsubsecheadstyle{\large\bfseries}
\setsubsubsecheadstyle{\normalsize\bfseries}

% -----------------------------------------------------------------------------

% Adjust spacing around sections
\setbeforesecskip{21pt}
\setaftersecskip{9pt}

% Adjust spacing around subsections
\setbeforesubsecskip{14pt}
\setaftersubsecskip{6pt}

% Adjust spacing around subsubsections
\setbeforesubsubsecskip{10pt}
\setaftersubsubsecskip{3pt}


==> preamble/tikz.tex <==

%!TEX root = ../main.tex

% -----------------------------------------------------------------------------

% Load TikZ and the necessary libraries
\usepackage{tikz}
\usetikzlibrary{angles,
                arrows,
                calc,
                chains,
                matrix,
                quotes,
                patterns,
                positioning,
                shapes,
                shapes.geometric,
                shapes.misc,
                decorations.markings,
                decorations.pathmorphing}

% -----------------------------------------------------------------------------

% Load pdfplots and set compatibility as recommended by pdfLaTeX
\usepackage{pgfplots}
\pgfplotsset{compat=1.14}

% -----------------------------------------------------------------------------

% Standalone package to include TikZ graphics as their own files
\usepackage{standalone}

% -----------------------------------------------------------------------------

% Define matplotlib colors for use with TikZ
\definecolor{color0}{HTML}{1F77B4}
\definecolor{color1}{HTML}{FF7F0E}
\definecolor{color2}{HTML}{2CA02C}
\definecolor{color3}{HTML}{D62728}
\definecolor{color4}{HTML}{9467BD}
\definecolor{color5}{HTML}{8C564B}
\definecolor{color6}{HTML}{E377C2}
\definecolor{color7}{HTML}{7F7F7F}
\definecolor{color8}{HTML}{BCBD22}
\definecolor{color9}{HTML}{17BECF}


==> preamble/typography.tex <==

%!TEX root = ../main.tex


% Make PDF searchable and copyable
% This needs to be loaded before fontenc
\usepackage{cmap}


% Prettier fonts
\usepackage[varg]{txfonts}
\usepackage[scaled=0.75]{beramono}


% Set the fontencoding to allow umlauts and better hyphenation
% textcomp is necessary for some additional glyphs, e.g. \textpm = ±
\usepackage[T1]{fontenc}
\usepackage{textcomp}


% Various mathematical symbols and environments
\usepackage{amsmath}
% \usepackage{amsthm}
\usepackage{amssymb}

% More (non-mathematical) symbols
\usepackage{fontawesome}


% Necessary to make \mathbb{1} work
\usepackage{bbold}


% More control over enumerate-environments, including inline enumerations
\usepackage[inline]{enumitem}


% Nicer fractions
\usepackage{nicefrac}



% Avoid clubs and widows
\clubpenalty=100000
\widowpenalty=100000


% Avoid short last lines in paragraphs
\setlength\parfillskip{0pt plus .4\textwidth}
\setlength\emergencystretch{2em}


% Define \escapeus{} to automatically escape underscores, e.g. in \hltt{}.
\makeatletter
\DeclareRobustCommand*{\escapeus}[1]{%
  \begingroup\@activeus\scantokens{#1\endinput}\endgroup}
\begingroup\lccode`\~=`\_\relax
   \lowercase{\endgroup\def\@activeus{\catcode`\_=\active \let~\_}}
\makeatother


% Define the \hltt{} command, which allows to typeset monospace text inside 
% a rounded  box for extra visibility / clarity.
\usepackage{tcolorbox}
\definecolor{hltextttgray}{rgb}{0.75, 0.75, 0.75}
\newtcbox{\hlbox}{nobeforeafter,
                  colframe=hltextttgray,
                  colback=hltextttgray!10,
                  boxrule=0.5pt,
                  arc=3pt,
                  boxsep=0pt,
                  left=2pt,
                  right=2pt,
                  top=1.5pt,
                  bottom=1.5pt,
                  tcbox raise base}
\newcommand{\hltt}[1]{\hlbox{\texttt{\escapeus{\vphantom{j}#1}}}}


% Load csquotes
% Always get correct (language-specific) quote character with \enquote{}
\usepackage{csquotes}


% Microtype
% Micro-typographical optimizations such as protrusion, kerning, ...
% Setting mostly taken from: http://www.khirevich.com/latex/microtype
\usepackage[activate={true, nocompatibility},
            final,
            tracking=true,
            kerning=true,
            spacing=false,
            factor=1100,
            stretch=10,
            shrink=10]{microtype}
\microtypecontext{spacing=nonfrench}
\SetTracking{encoding={*}, shape=sc}{40}
\SetProtrusion{encoding={*},family={kpfonts},series={*},size={6,7}}
              {1={ ,750},2={ ,500},3={ ,500},4={ ,500},5={ ,500},
               6={ ,500},7={ ,600},8={ ,500},9={ ,500},0={ ,500}}


% Correctly typeset "dx" in integrals with \dif x
%\usepackage{commath}
\newcommand{\dif}{\ensuremath{\:d}}


% Load siunitx
% This ensures correct typography for physical units (e.g. proper spacing)
% Syntax: \SI{number}{\unit}
\usepackage{siunitx}
\sisetup{range-units = single,
         range-phrase = {-},
         separate-uncertainty = true,
         multi-part-units = brackets,
         product-units = brackets,
         detect-weight = true,
         binary-units = true,
         per-mode = symbol,
         mode = text}

% Define custom units
\let\sun\odot
\DeclareSIUnit \solarmass {\ensuremath{M_\sun}}
\DeclareSIUnit \parsec {pc}
\DeclareSIUnit \year {yr}

